Left-invariant optimal control problems on Lie groups

Left-invariant optimal control problems on Lie groups form an important class of problems with big symmetry group. They are interesting from the theoretical point of view since they often can be completely studied, and general features can be investigated on these model problems. In particular, problems on nilpotent Lie groups give a fundamental nilpotent approximation of general problems. Left-invariant problems also often arise in applications: in classical and quantum mechanics, geometry, robotics, models of vision and image processing. This work aims to review the main notions, methods and results for left-invariant optimal control problems on Lie groups. The main attention is paid to description of extremal trajectories and their optimality, cut time and cut locus, optimal synthesis. Bibliography: 238 titles.

==> bib_old.tex <==
\begin{thebibliography}{99}\addcontentsline{toc}{section}{Список литературы}

\subsection*{Книги по теории управления, вариационному исчислению и неголономной геометрии}
\bibitem{notes}
А.А.~Аграчев, Ю. Л. Сачков,  
%{\em Geometric control theory}, Fizmatlit, Moscow 2004; English transl.
{\em Геометрическая теория управления},
Физматлит, 2005.

\bibitem{ATF}
В.М. Алексеев, В.М. Тихомиров, С.В. Фомин,  
%{\em Geometric control theory}, Fizmatlit, Moscow 2004; English transl.
{\em Оптимальное управление},
Физматлит, 2005.

\bibitem{griffith}
Ф. Гриффитс, {\em  Внешние дифференциальные системы и вариационное исчисление},
М.: Мир, 1986. 

\bibitem{monroy}
Anzaldo-Menezes A., Monroy-P\'erez F.
Charges in magnetic fields and sub-Riemannian geodesics//
Contemporary trends in nonlinear geometric control theory and its
applications. Singapore:  World Scientific, 2002. P.~183--202.



\bibitem{li_canny}
Li Z., Canny J.
Motion of two rigid bodies with rolling constraint//
IEEE Trans. Robot. Automat. (1). 1990. V.~6. P.~62--72.


\bibitem{cdc99}
Agrachev A.\,A., Sachkov Yu.L.
An intrinsic approach to the control of rolling bodies//
Proceedings of the 38-th
IEEE Conference on Decision and Control, Phoenix, Arizona, USA, December
7--10, 1999. V.~1. P.~431--435.

\bibitem{marigo_bicchi}
Marigo A., Bicchi A.
Rolling bodies with regular surface: the holonomic case//
 Differential geometry and control: Summer Research Institute
on Differential Geometry and Control,  Univ.
Colorado, Boulder, June 29--July 19, 1997, / ed.~G.~Ferreyra et al. Providence, RI: Amer. Math.~Soc., 1999. P.~241--256 (Proc.~Sympos.~Pure Math. V.~64).



\bibitem{versh_gersh}
Вершик А.М., Гершкович В.Я.
{\em Неголономные динамические системы. Геометрия распределений и вариационные
задачи}.
Итоги науки и техники: Современные проблемы математики, Фундаментальные
направления, т. 16, ВИНИТИ, Москва, 1987, 5--85.

\bibitem{versh_gersh2}
Вершик А.М., Гершкович В.Я.
{\em Неголономные задачи и геометрия распределений}.
Добавление к книге \cite{griffith}, с. 318--349.

\bibitem{zelikin}
М.И. Зеликин, {\em Оптимальное управление и вариационное исчисление}, М.: URSS, 2014.

\bibitem{PGBM}
Понтрягин Л.\,С., Болтянский В.\,Г., Гамкрелидзе Р.\,В., Мищенко Е.\,Ф.
{\em Математическая теория оптимальных процессов},
М.: Наука, 1961.

\item	Сачков Ю.Л. Теория управления на группах Ли, {\em Современная математика. Фундаментальные направления}, 2007, т. 27, 5--59.

\bibitem{mono}
Сачков Ю.Л. {\em Управляемость и симметрии инвариантных систем на группах Ли и однородных пространствах}. ---М.: Физматлит, 2007.

\bibitem{intro}
Сачков Ю.Л. {\em Введение в геометрическую теорию управления}, в печати.

\bibitem{cime}
Agrachev A.A.,  
Geometry of optimal control problems and Hamiltonian systems. In: Nonlinear and Optimal Control Theory,  Lecture Notes in Mathematics. CIME, 1932, Springer Verlag,  2008, 1-59.

\bibitem{agrachev_open}
A. A. Agrachev. {\em Some open problems}, pp. 1–13. Springer International
Publishing, Cham, 2014.

\bibitem{ABB_book}
A. Agrachev, D. Barilari, U. Boscain, {\em A Comprehensive Introduction to
sub-Riemannian Geometry from Hamiltonian viewpoint}, Cambridge Studies in Advanced Mathematics, Cambridge Univ. Press, 2019

\bibitem{agr_gam}
A. A. Agrachev and R. V. Gamkrelidze, Symplectic geometry for optimal control, Nonlinear controllability
and optimal control, Monogr. Textbooks Pure Appl. Math., vol. 133, Dekker, New York, 1990, pp. 263--
277.

\bibitem{SRG} A.~Bellaiche, J.~Risler, Eds., Sub-Riemannian geometry.
Birkh\"aser, Progress in Math., 1996, v.144

\bibitem{bloch} 
A. Bloch,
{\em Nonholonomic Mechanics and Control},
Interdisciplinary Applied Mathematics, Volume 24, Springer, 2003.

\item U.~Boscain, B.~Piccoli, Optimal synthesis for control
systems on 2-D manifolds. Springer SMAI, v.43, 2004.

\bibitem{sussmann}
R.~W.~Brockett, R.~S.~Millman, H.~J.~Sussmann, Eds.,
Differential geometric conrol theory. Birkh\"auser Boston, 1983

\bibitem{capogna}
Luca Capogna, Donatella Danielli, Scott D. Pauls, and Jeremy T. Tyson.
{\em An introduction to the Heisenberg group and the sub-Riemannian
isoperimetric problem}, volume 259 of Progress in Mathematics.
Birkh\"auser Verlag, Basel, 2007.

\bibitem{euler}
Euler L., \textit{Methodus inveniendi lineas curvas maximi minimive proprietate gaudentes, sive Solutio problematis isoperimitrici latissimo sensu accepti}, Lausanne, Geneva, 1744.


\bibitem{isidori}
A.~Isidori,
{\em Nonlinear control systems: an introduction},
Springer-Verlag,  1985.


\item B.~Jakubczyk, W.~Respondek, Eds.,
Geometry of feedback and optimal control.
Marcel Dekker, 1998

\item
Fr\'ed\'eric Jean. {\em Control of nonholonomic systems: from sub-Riemannian
geometry to motion planning}. SpringerBriefs in Mathematics. Springer,
Cham, 2014.

\bibitem{jurd_book}
V.~Jurdjevic,
{\em Geometric Control Theory},
Cambridge University Press, 1997.

\bibitem{jurd16}
Velimir Jurdjevic. Optimal control and geometry: integrable systems.
Cambridge University Press, Cambridge, 2016.


\bibitem {montgomery_book}
R. Montgomery, {\em A tour of subriemannnian geometries, their geodesics and applications}, Amer. Math. Soc., 2002


\bibitem{nijmeijer_vanderschaft}
H.~Nijmeijer, A. ~van der Schaft,
{\em Nonlinear dynamical control systems},
Springer-Verlag, 1990.

\bibitem{rifford}
L. Rifford. {\em Sub-Riemannian geometry and Optimal Transport}.
SpringerBriefs in Mathematics, 2014.

\bibitem{sontag}
E.\,D.~Sontag,
{\em Mathematical control theory : deterministic finite dimensional systems},
Springer-Verlag, 1990.


\bibitem{sus_nonlin} 
H.~J.~Sussmann, Ed.,
Nonlinear controllability and optimal control.
Marcel Dekker, 1990

\bibitem{zelikin_borisov}
M.\,I.~Zelikin, V.\,F.~Borisov,
{\em Theory of chattering control with applications to astronautics, robotics,
economics, and engineering},
Basel: Birkhauser, 1994.



\subsection*{Другие книги}
\bibitem{tikhomirov_stories}
В.М. Тихомиров, {\em Рассказы о максимумах и минимумах}, М.: МЦНМО, 2006

\bibitem{whit_watson}
Э.Т. Уиттекер, Дж.Н. Ватсон,
{\em 
Курс современного анализа},
М.: УРСС, 2002.

\bibitem{warner}
Ф. Уорнер,
{\em 
Основы теории гладких многообразий и групп Ли},
М.: Мир, 1987.

\bibitem{hadamard}
Krantz~S.~G., Parks~H.~R., \textit{The Implicit Function Theorem: History, Theory, and Applications}, Birkauser, 2001.

\bibitem{lawden}
D. F. Lawden,  {\em  Elliptic Functions and Applications}, Springer, 1989

\bibitem{akhiezer}
Н.И. Ахиезер,
{\em 
Элементы теории эллиптических функций},
М.: Наука, 1970.

\bibitem{vilenkin}
Н.Я, Виленкин, {\em Специальные функции и теория представлений групп}, М.: Мир, 1965. 

\bibitem{lan_liv}
Ландау Л. Д., Лифшиц Е. М. Механика. — 5-е изд., стереотип. — М.: ФИЗМАТЛИТ, 2012. — 224 с.

\subsection*{Субриманова задача на группе Гейзенберга}
\bibitem{brock}
Brockett R.
Control theory and singular Riemannian geometry//
In: New Directions in Applied Mathematics, (P.~Hilton and G.~Young eds.),
Springer-Verlag, New York, 11--27, 1982.

\subsection*{Задача Эйлера об эластиках}

\bibitem{el_AiT}
А.А.Ардентов, Ю.Л.Сачков. Решение задачи Эйлера об эластиках.  {\em Автоматика и телемеханика}, 2009, No.  4, 78--88.



\bibitem{love}
{\sl Ляв~А.} Математическая теория упругости. Москва-Ленинград:
ОНТИ, 1935.

\bibitem{el_dan}
Сачков Ю.Л. Оптимальность эйлеровых эластик, {\em Доклады Академии Наук}, том 417, No. 1, ноябрь 2007, С. 23--25.

\bibitem{euler_rus}
{\sl Эйлер~Л.} Метод нахождения кривых линий, обладающих
свойствами максимума или минимума, или решение изопериметрической
задачи, взятой в самом широком смысле, Леонарда Эйлера,
королевского профессора и члена Императорской Петербургской
Академии Наук. Приложение I. <<Об упругих кривых>>.
Москва-Ленинград: ГТТИ, 1934. С. 447-572.

\bibitem{el_stable}
	Сачков Ю.Л., Левяков С.В. Устойчивость инфлексионных эластик, центрированных в вершинах или точках перегиба, {\em Труды МИАН}, 2010,  T. 271, 187--203.
	
\bibitem{antman}
S.S.Antman,
The influence of elasticity on analysis: Modern developments,
{\em Bulletin American Math. Society}, 1983, v. 9, No. 3, 267--291.

\bibitem{DBernoulli}
D.Bernoulli, 26th letter to L. Euler (October, 1742), In: Fuss, {\em Correspondance math\'ematique et physique}, t.2, St. Petersburg, 1843.

\bibitem{JBernoulli}
J.Bernoulli,
V\'eritable hypoth\`ese de la r\'esistance des solides, avec la demonstration de la corbure des corps qui font ressort,
In: {\em Collected works}, t.2, Geneva, 1744.
	

\bibitem{birkhoff64}
{\sl Birkhoff~G., de Boor~C.R.} Piecewise polynomial interpolation
and approximation // Approximation of Functions. Proc. Sympos.
General Motors Res. Lab., 1964. Elsevier. Amsterdam: 1965. P.
164-190.

\bibitem{born}
Max Born. Stabilitat der elastischen Linie in Ebene und Raum.
Preisschrift Und Dissertation, 1: 5–101, 1906.	
	
\bibitem{jurd_noneuclid}
V.Jurdjevic,
Non-Euclidean elastica,
{\em Am. J. Math.}, v. 117 (1995), 93--125.

\bibitem{levien}
{\it Levien R.} The elastica: a mathematical history // Technical Report No. UCB\slash EECS-2008-103,	2008, P. 1--25.



\bibitem{manning96}
R.S.Manning, J.H.Maddocks, J.D.Kahn,
A continuum rod model of sequence-dependent DNA structure,
{\em J. Chem. Phys.} v. 105 (1996), 5626--5646.

\bibitem{manning98}
R.S.Manning, K.A.Rogers, J.H.Maddocks,
Isoperimetric conjugate points with application to the stability of DNA minicircles,
{\em Proc. R. Soc. Lond. A}, v. 454 (1998), 3047--3074.

\bibitem{el_SE2}
A. Mashtakov, A. Ardentov, Yu. Sachkov, Relation between Euler’s elasticae and sub-Riemannian geodesics on SE(2), {\em Regular and Chaotic Dynamics}, December 2016, Volume 21, Issue 7, pp 832--839.	

\bibitem{mumford}
D.Mumford,
Elastica and computer vision, In:
{\em Algebraic geometry and its applications},
C.L.Bajaj, Ed., Springer-Verlag, New-York, 1994, 491--506.

\bibitem{saalchutz}
L.Saalsch\"utz,
{\em Der belastete Stab}, Leipzig, 1880.
	
\bibitem{el_max}
Yu. L. Sachkov,
Maxwell strata in Euler's elastic problem,
Journal of Dynamical and Control Systems,
Vol. 14 (2008), No. 2  (April), pp. 169--234. 


\bibitem{el_conj}
Yu. L. Sachkov,
Conjugate points in Euler's elastic problem,
{\em Journal of Dynamical and Control Systems}, vol. 14 (2008), No. 3 (July).

\bibitem{el_closed}
Yu. Sachkov, Closed Euler Elasticae, {\em Proceedings of the Steklov Institute of Mathematics}, V. 278 (2012), 218--232.

\bibitem{el_cut}
Yu. L. Sachkov, E.Sachkova,
Exponential mapping in Euler's elastic problem,
{\em Journal of Dynamical and Control Systems}, Vol. 20 (2014),    No. 4, 443--464.

\bibitem{timoshenko}
S.Timoshenko,
{\em History of Strength of Materials},
McGraw-Hill, New-York, 1953.

\bibitem{truesdell}
C.Truesdell,
The Influence of Elasticity on Analysis: The Classic Heritage,
{\em Bulletin American Math. Society}, 1983, v. 9, No. 3, 293--310.

\bibitem{Greenhill}
A. G. Greenhill, 
{\em The applications of elliptic functions} (New York, Macmillan, 1892).

\bibitem{Frisch}
R. Frisch Fay, 
{\em Flexible Bars}, Butterworths, London (1962).

\bibitem{Bisshopp}
K.E. Bisshopp, D.C. Drucker, Large deflection of cantilever beams. 
{\em Quart. Appl. Math.} 3 (1945) 272-275.

\bibitem{Lardner}
T. J. Lardner, A note on the elastica with large loads, 
{\em Int. J. Solids Struct.}, Vol. 21. No. 1. pp. 21-26, I985.

\bibitem{Wang}
C. Y. Wang, Post-buckling of a clamped-simply supported elastica, 
{\em Int. J. Non-Linear Mechanics}, Vol. 32. No. 6, pp. I 115-l 122, 1997.

\bibitem{Panayotounakos}
D. E. Panayotounakos, P. S. Theocaris, Analytic solutions for nonlinear differential equations describing the elastica of straight bars : Theory, 
{\em Journal of the Franklin Institute}, Vol. 325, No. 5, pp. 621433, 1988.

\bibitem{Seide}
P. Seide. Large deflections of a simply supported beam subjected to moment at one end, 
{\em Trans. ASME, J. Appl. Mech.}, Vol. 51, 519-525, 1984.

\bibitem{Naschie}
M. S. El Naschie, Thermal initial post buckling of the extensional elastica, 
{\em Int. J. Mechanical Science}, 1976, Vol. 18, pp. 321-324.

\bibitem{Stampouloglou}
I. H. Stampouloglou, E. E. Theotokoglou, P. N. Andriotaki , Asymptotic solutions to the non-linear cantilever elastica, 
{\em Int. J. Non-Linear Mechanics}, 40 (2005) 1252 - 1262.

\bibitem{Glassmaker}
N. J. Glassmaker, C. Y. Hui, Elastica solution for a nanotube formed by self-adhesion of a folded thin film, 
{\em J. Appl. Physics}, V. 96, N. 6, 3429-3434.

\bibitem{Tang}
T. Tang, N. J. Glassmaker, On the inextensible elastica model for the collapse of nanotubes, {\em Mathematics and Mechanics of Solids}, 2009, doi:10.1177/1081286509105923.

\bibitem{Mikata}
Y. Mikata, Complete solution of elastica for a clamped-hinged beam, and its applications to a carbon nanotube, {\em Acta Mechanica} 190, 133-150 (2007).

\bibitem{Heijden}
van der Heijden, G.H.M., Neukirch, S., Goss, V.G.A., Thompson, J.M.T.: Instability and self-contact phenomena in the writhing of clamped rods. 
{\em Int. J. Mech. Sci.} 45, 161-196 (2003).


\subsection*{Субриманова задача на группе $\SE(2)$}

\bibitem{max_sre}
I. Moiseev, Yu. L. Sachkov,
Maxwell strata in sub-Riemannian problem  on the group of motions of a plane,
{\em ESAIM: COCV}, 16 (2010), 380--399.

\bibitem{cut_sre1}
Yu. L. Sachkov,
Conjugate and cut time in the sub-Riemannian problem on the group of motions of a 
plane, {\em ESAIM: COCV}, 16 (2010), 1018--1039.

\bibitem{cut_sre2}
Yu. L. Sachkov,
Cut locus and optimal synthesis in the sub-Riemannian problem  on the group of motions of a 
plane, {\em ESAIM: COCV}, 17 (2011), 293--321.

\bibitem{bicycle}
A. Ardentov,  G. Bor, E. Le Donne,  R. Montgomery, Yu. Sachkov,
 Bicycle paths, elasticae and sub-Riemannian geometry, 
{\em Nonlinearity},  принята к публикации. 

\bibitem{se2_GO}
Ю.Л. Сачков, Однородные субримановы геодезические на группе движений плоскости, {\em направлена для  публикации}.

\subsection*{Задача о качении сферы по плоскости}

\bibitem{s2r2}
Маштаков А.П., Сачков Ю.Л.,  Экстремальные траектории и асимптотика времени Максвелла в задаче об оптимальном качении сферы по
плоскости, {\em Математический сборник} (2011),  Т.  202, No. 9, C. 97--120.

\bibitem{s2r2_sym}
	Сачков Ю.Л. Симметрии и страты Максвелла и симметрии в задаче об оптимальном качении сферы по плоскости, {\em Мат. Сборник}, 2010,  T. 201, N 7, С. 99--120.

\bibitem{arthur_walsh} A.M. Arthurs, G.R.Walsh, On the Hammersley’s minimum problem for a rolling
sphere, {\em Math. Proc. Cambridge Phil. Soc.}, 99 (1986), 529–534.

\bibitem{bicchi_prat_sast}
Bicchi A., Prattichizzo D., Sastry S., Planning motions of rolling surfaces// IEEE Conf. on Decision and Control, 1995

\bibitem{hammersley}
J.M. Hammersley, Oxford commemoration ball, Probability, Statistics and Analysis
(London Math. Soc. lecture notes), 79 (1983), 112–142.



\bibitem{jurd_ball} 
V. Jurdjevic, The geometry of the plate-ball problem, {\em Arch. Rat. Mech. Anal.}, 124
(1993), 305–328.

\bibitem{roll_besch}
И. Ю. Бесчастный,
Об оптимальном качении сферы с прокручиванием, без проскальзывания, {\em Матем. сб.}, 205:2 (2014),  3–38

%\bibitem{li_canny}
%Li Z., Canny J.,  Motion of two rigid bodies with rolling constraint//
%IEEE Trans. on Robotics and Automation, 1(6), pp. 62--72, 1990

%\bibitem{marigo_bicchi}
%Marigo A., Bicchi A., Rolling bodies with regular surface: the holonomic case, 
%in book: ``Differential geometry and control: Summer Research Institute
%on Differential Geometry and Control'', publ. Univ. Colorado, Boulder, G.~Ferreyra et al. Eds, pp. 241--256,
%1999

\subsection*{Субриманова задача на группе Энгеля}
\bibitem{vesrh_gran91}
***
Вершик А.М., Граничина О.А.,  Редукция неголономных вариационных задач к изопериметрическим и связности в главных расслоениях, {\em Мат. заметки} (1991), Т.  202, No. 11, C. 37--44.

\bibitem{engel}
Ардентов А.А., Сачков Ю.Л.,  Экстремальные траектории в нильпотентной субримановой задаче на группе Энгеля, {\em Мат. сборник} (2011), Т.  49, No. 5, C. 31--54.

\bibitem{engel_dan}	А.А.Ардентов, Ю.Л.Сачков, Множество разреза в субримановой задаче на группе Энгеля, {\em Доклады Академии Наук}, Выпуск 6, 2018, Том 478,  623--626.

\bibitem{engel_conj}
Ardentov, A.\,A. and Sachkov, Yu.\,L., Conjugate points in nilpotent sub-Riemannian problem on the Engel group, \textit{Journal of Mathematical Sciences}, 2013, vol.\,195, no.\,3, pp.\,369--390.

\bibitem{engel_cut}
Ardentov, A.\,A. and Sachkov, Yu.\,L., Cut time in sub-Riemannian problem on Engel group, \textit{ESAIM: COCV}, 2015, vol.\,21, no.\,4, pp.\,958--988.

\bibitem{engel_synth}
A.A. Ardentov, Yu. L. Sachkov,
Maxwell Strata and Cut Locus in the Sub-Riemannian Problem on the Engel Group, Regular and Chaotic Dynamics, December 2017, Vol. 22, Issue 8, pp 909--936.

\bibitem{engel_sphere}
Yu. L. Sachkov, On the structure of Engel sub-Riemannian sphere, {\em в работе}.

\subsection*{Субриманова задача на группе Картана}

\bibitem{cartan1910}
E.~Cartan,
L\`es systemes de Pfaff a cinque variables et l\`es equations aux
derivees partielles du second ordre,
{\em Ann. Sci. \`Ecole Normale} {\bf 27} (1910), 3: 109--192.


\bibitem{dido_exp}
Сачков Ю.Л., Экспоненциальное отображение в обобщенной задаче Дидоны, {\em Математический сборник}, 2003, 194 (9),  63--90.

\bibitem{max1}
Сачков Ю.Л.  Дискретные симметрии в обобщенной задаче Дидоны, {\em Мат. Сборник}, 2006, T. 197, N 2, S. 95--116.


\bibitem{max2}
Сачков Ю.Л. Множество Максвелла в обобщенной задаче Дидоны, {\em Мат. Сборник}, 2006, Т. 197,  № 4, С. 123--150.

\bibitem{max3}
Сачков Ю.Л. Полное описание стратов Максвелла в обобщенной задаче Дидоны, {\em Мат. Сборник}, 2006,  T. 197, N 6, С. 111--160.

\bibitem{brock_dai}
Brockett R., Dai L.
Non-holonomic kinematics and the role of el\-lip\-tic functions in
constructive controllability//
In: Nonholonomic Motion Planning, Z.~Li and J.~Canny, Eds.,
Kluwer, Boston, 1993, 1--21.

\bibitem {symmetry}
Yu. L. Sachkov, Symmetries of flat rank two distributions and sub-Riemannian structures, {\em Transactions of the AMS}, 2004, 2, 457-494

\bibitem{cartan_conj}
Yu. L. Sachkov, Conjugate time in the  sub-Riemannian problem on the  Cartan group, {\em Journal of Dynamical and Control Systems}, accepted.

\bibitem{cartan_cut}
A. Ardentov, E. Hakavuori,  Cut time in the  sub-Riemannian problem on the  Cartan group, {\em in preparation}.

\subsection*{Субриманова задача на группе $\SH(2)$}

\bibitem{sh2_1}
Y.A.Butt, A.I. Bhatti, Yu. L. Sachkov,
Parametrization of Extremal Trajectories in Sub-Riemannian Problem on Group of
Motions of Pseudo Euclidean Plane,
{\em Journal of Dynamical and Control Systems},  
Vol. 20 (2014), No. 3 (July), 341--364.

\bibitem{sh2_2}
Y.A.Butt, A.I. Bhatti, Yu. L. Sachkov,
Maxwell strata and conjugate points in sub-Riemannian problem on the group $\SH(2)$,
{\em Journal of Dynamical and Control Systems}, 22 (2016),  747--770

\bibitem{sh2_3}
Y.A.Butt, A.I. Bhatti, Yu. L. Sachkov,
Cut Locus and Optimal Synthesis in Sub-Riemannian Problem on the Lie
Group $\SH(2)$,
{\em Journal of Dynamical and Control Systems},  23 (2017), 155--195

\subsection*{Римановы задачи на группах $\SO(3)$, $\SU(2)$, $\SL(2)$ и  $\PSL(2)$}

\bibitem{bates-fasso}
{\it L.~Bates, F.~Fass\`{o}.} The Conjugate Locus for the Euler Top. I. The Axisymmetric Case. //
International Mathematical Forum. 2007. 2, 43. 2109--2139.

\bibitem{sakai}
{\it T.~Sakai.} Cut loci of Berger's sphere. // Hokkaido Mathematical Journal. 1981. 10. 143--155.


\bibitem{so3_sl2_dan}
	А.В.Подобряев, Ю.Л.Сачков, Левоинвариантные симметричные римановы задачи на группах собственных движений плоскости Лобачевского и сферы,  {\em Доклады Академии Наук}, 2017, 473, No. 6, с. 640--642
	
\bibitem{so3}
A.Podobryaev, Yu. L. Sachkov,
Cut locus of a left invariant Riemannian metric on $\SO(3)$ in the axisymmetric case,
{\em Journal of Geometry and Physics},    110 (2016) 436--453.

\bibitem{diamsu2}
А. В. Подобряев, Диаметр сферы Берже, Матем. заметки, 103:5 (2018), 779–784



\bibitem{sl2}
A.Podobryaev, Yu. L. Sachkov,
Symmetric Riemannian Problem on the Group of Proper Isometries of Hyperbolic Plane, J Dyn Control Syst (2018) 24: 391 

\subsection*{Субриманова задача в плоском случае Мартине}

\bibitem{martinet}
A.Agrachev, B. Bonnard, M. Chyba, I. Kupka,
Sub-Riemannian sphere in Martinet flat case. J. ESAIM: Control, Optimisation and Calculus of Variations, 1997, v.2,
377--448 

\subsection*{$\exp$-$\log$  категория}
\bibitem{dries}
L.V.D. Dries, A. Macintyre, D. Marker, The elementary theory of restricted analytic fields with exponentiation, {\em Annals of Mathematics}, 140, 1994, 183--205.
\bibitem{lion}
J.M. Lion, J.P. Rolin, Th\'eor\`emes de pr\'eparation pur les fonctions logarithmo-exponentielles, {\em Annales de l'Institut Fourier}, 47, 1997, 859--884.

\subsection*{Субриманова задача на двухступенных свободных нильпотентных группах Ли}
\bibitem{brock80}
R.W. Brockett. “Control theory and singular Riemannian geometry”,
New Directions in Applied Mathematics, Occasion of the Case Centennial
Celebration (April 25/26, 1980), eds. P.J. Hilton, G.S. Young, 1982,
pp. 11–27.

\bibitem{gaveau}
B. Gaveau. “Principe de moindre action, propagation de la chaleur et
estimees sous elliptiques sur certains groupes nilpotents”, Acta Mathematica,
139 (1977), pp. 95–153.

\bibitem{liusus}
W.S. Liu, H. Sussmann, 
Shortest paths for sub-Riemannian metrics on rank-2 distributions, 
 Memoirs of the American Mathematical Society, No. 564, Vol. 118, November 1995

\bibitem{monroy_meneses}
F. Monroy-Pérez, A. Anzaldo-Meneses. “The step-2 nilpotent $(n, n(n + 1)/2)$
sub-Riemannian geometry”, Journal of Dynamical and Control Systems, 12:2
(2006), pp. 185–216.

\bibitem{montanari_morbidelli}
A. Montanari, D. Morbidelli. On the sub-Riemannian cut locus in a model of free
two-step Carnot group, Calc. Var. 56, 36 (2017), 1 - 26.

\bibitem{myasn36}
O. Myasnichenko. “Nilpotent $(3, 6)$ sub-Riemannian problem”, Journal of
Dynamical and Control Systems, 8:4 (2002), pp. 573–597

\bibitem{myasn06}
Oleg Myasnichenko. Nilpotent $(n, n(n + 1)/2)$ sub-Riemannian
problem. J. Dyn. Control Syst., 12(1): 87–95, 2006.

\bibitem{rizzi_serres}
L. Rizzi, U. Serres. On the cut locus of free, step two Carnot groups, Proc. Amer. Math. Soc. 145 (2017), 5341-5357

\bibitem{ledonne_sard}
E. Le Donne, R. Montgomery, A. Ottazzi, P. Pansu, D.Vittone,
Sard property for the endpoint map on some Carnot groups,
Annales de l'Institut Henri Poincar\'e C, Analyse non lin\'eaire
Volume 33, Issue 6, November–December 2016, Pages 1639-1666


\subsection*{Двухступенные  субримановы задачи коранга 1 и 2}
\bibitem{corank1}
A. Agrachev, D. Barilari, U. Boscain, On the Hausdorff volume in sub-Riemannian geometry, 
{\em Calculus of variations and partial differential equations}, 
43 (2012), 3--4, 355--388.

\bibitem{corank2}
D. Barilari, U. Boscain, J.-P. Gauthier,
On 2-step, corank 2 nilpotent sub-Riemannian metrics,
SIAM Journal on Control and Optimization 50 (2012), 1:559--582


\subsection*{Симметричные субримановы задачи на группах $\SO(3)$, $\SU(2)$, и $\SL(2)$}
\bibitem{gersh84}
В.Я. Гершкович, Вариационная задача с неголономной связью на $\SO(3)$. --- В сб.: Новое в глобальном анализе. --- Воронеж: Изд-во ВГУ, 1984, с. 149--152.

\bibitem{versh_gersh86}
***
А. М. Вершик, В. Я. Гершкович, “Геодезический поток на $\SL(2,\R)$ с неголономными ограничениями”, Записки научных семинаров ЛОМИ / Акад. наук СССР, Мат. ин-т им. В. А. Стеклова, Ленингр. отд-ние. - Л. : Наука, Т. 155 : Дифференциальная геометрия, группы Ли и механика : 7 : сб. работ / под ред. Л. Д. Фаддеева. – 1986, 7–17

\bibitem{ber01}
В. Н. Берестовский, И. А. Зубарева, “Формы сфер специальных неголономных левоинвариантных внутренних метрик на некоторых группах Ли”, Сибирский математический журнал, 42:4 (2001), 731–748

\bibitem{ber151}
	В. Н. Берестовский, “(Локально) кратчайшие специальной субримановой метрики на группе Ли SO0(2,1)”, Алгебра и анализ, 27:1 (2015), 3–22

\bibitem{BZ15a}
В. Н. Берестовский, И. А. Зубарева, “Геодезические и кратчайшие специальной субримановой метрики на группе Ли SO(3)”, Сиб. матем. журн., 56:4 (2015), 762–774

\bibitem{BZ15b} 
В. Н. Берестовский, И. А. Грибанова, “Субриманово расстояние в группах Ли SU(2) и SO(3)”, Матем. тр., 18:2 (2015), 3–21

\bibitem{BZ16}
В. Н. Берестовский, И. А. Зубарева, “Геодезические и кратчайшие специальной субримановой метрики на группе Ли SL(2)”, Сиб. матем. журн., 57:3 (2016), 527–542

\bibitem{BZ16_2}
В. Н. Берестовский, И. А. Зубарева, “Субриманово расстояние в группе Ли SO0(2,1)”, Алгебра и анализ, 28:4 (2016), 62–79

\bibitem{BZ17}
В. Н. Берестовский, И. А. Зубарева, “Субриманово расстояние в группе Ли SL(2)”, Сиб. матем. журн., 58:1 (2017), 22–35 

\bibitem{boscain_rossi}
U. Boscain, F. Rossi. “Invariant Carnot–Caratheodory metrics on 
$S^3$, $\SO(3)$, $\SL(2)$ and lens spaces”, SIAM J. Control Optim., 47 (2008), pp. 1851–1878

\bibitem{chang_markina_vasiliev}
D.Ch. Chang, I. Markina, A. Vasiliev,
Sub-riemannian geodesics on the 3-sphere,
{\em Compl. anal. oper. theory}, 3 (2009), 361--377.

\bibitem{BS16}
И. Ю. Бесчастный, Ю. Л. Сачков, “Геодезические в субримановой задаче на группе SO(3)”, Матем. сб., 207:7 (2016), 29–56 

\subsection*{Субримановы задачи с неинтегрируемым геодезическим потоком}

\bibitem{LS2017}		Л. В. Локуциевский, Ю. Л. Сачков, Неинтегрируемость по Лиувиллю субримановых задач на свободных группах Карно глубины 4,  {\em Доклады Академии Наук}, 2017, т. 95, no. 3, С. 211–213.

\bibitem{LS2018}	
Л. В. Локуциевский, Ю. Л. Сачков, Об интегрируемости по Лиувиллю субримановых задач на группах Карно глубины 4 и больше, {\em Матем. сб.}, 209:5 (2018), 74–119 


\bibitem{SS17}
Ю. Л. Сачков, Е.Ф. Сачкова, Вырожденные анормальные траектории в субримановой задаче с вектором роста (2,3,5,8), Дифференциальные уравнения, 2017, 3, 362--374.

\bibitem{gole_karidi}
Gol\'e, C., Karidi, R. A note on Carnot geodesics in nilpotent Lie groups. {\em Journal of Dynamical and Control Systems} 1, 535–549 (1995).

\bibitem{borisov}
Bizyaev I. A.,  Borisov A. V.,  Kilin A. A.,  Mamaev I. S., Integrability and Nonintegrability of Sub-Riemannian Geodesic Flows on Carnot Groups, Regular and Chaotic Dynamics, 2016, vol. 21, no. 6, pp. 759-774

\subsection*{Классификации левоинвариантных субримановых задач}
\bibitem{versh_gersh88}
***
А. М. Вершик, В. Я. Гершкович, Геометрия неголономной сферы трехмерных групп Ли, Геометрия и теория особенностей в нелинейных уравнениях. Новое в глобальном анализе, 61—75. Воронеж, 1987. Перевод на англ. язык:  Lect. Notes in Math. 1334, 309-331 (1988).

\bibitem{FG}
Elisha Falbel and Claudio Gorodski. Sub-Riemannian homogeneous
spaces in dimensions 3 and 4. Geom. Dedicata, 62(3): 227–252, 1996.

\bibitem{agr_bar}
A.Agrachev, D. Barilari, 
Sub-Riemanian structures on 3D Lie groups. {\em J. Dynamical and Control Systems}, 2012, v.18, 21--44

\bibitem{almeida1}
D. Almeida, Sub-riemannian symmetric spaces of engel type, {\em Mat. contemp.}, 17 (1998), pp. 45–58.


\bibitem{almeida2}
D. Almeida, Sub-riemannian homogeneous spaces of engel type, {\em J. Dynamic. and Control Syst.}, 20 (2014), pp. 149–
166.

\bibitem{BM}
I. Beschastnyi, A. Medvedev, Left-invariant Sub-Riemannian Engel structures: abnormal geodesics and integrability, 	arXiv:1611.03634 [math.DG]


\subsection*{Левоивариантные субфинслеровы задачи}
\bibitem{ADS19}
Ардентов А.А., Э. Ле Донне, Сачков Ю.Л., Субфинслеровы геодезические на группе Картана, Regular and Chaotic Dynamics, 2019,  vol. 24, no. 1, pp. 36-60

\bibitem{AS19_1}
Ардентов А.А., Э. Ле Донне, Сачков Ю.Л., Экстремальные траектории в субфинслеровой задаче на группе Картана, Труды МИАН, т. 304 (2019), 49–67.

\bibitem{AS19_2}
Ардентов А.А., Сачков Ю.Л., Субфинслерова задача на группе Картана, Доклады Академии Наук, 2019, 484, No. 2, 138-141

\bibitem{AS19_3}
Ардентов А.А., Сачков Ю.Л., Субфинслеровы структуры на группе Энгеля, Доклады Академии Наук, 2019, 485, No. 4, 395—398

\bibitem%[Ber89a]
{b1}
Берестовский В.Н., \emph{Однородные многообразия с внутренней метрикой. {II}}, Сибирский математический журнал, \textbf{30} (1989), no.~2, 14--28,
  225.

\bibitem%[Ber89b]
{b2}
Берестовский В.Н., \emph{О структуре однородных локально компактных пространств с внутренней метрикой}, Сибирский математический журнал, \textbf{30} (1989), no.~1, 23--34.

\bibitem{ber94}
В. Н. Берестовский, “Геодезические неголономных левоинвариантных внутренних метрик на группе Гейзенберга и изопериметриксы плоскости Минковского”, Сиб. матем. журн., 35:1 (1994), 3–11

\bibitem{convex}
Локуциевский Л.В. 
Выпуклая тригонометрия с приложениями к субфинслеровой геометрии // Матем. сб. 2019. Т. 210. № 8. С. 120--148.

\bibitem%[BBLS17]
{BBLDS}
Davide Barilari, Ugo Boscain, Enrico {L}{e Donne}, and Mario Sigalotti,
  \emph{Sub-{F}insler structures from the time-optimal control viewpoint for
  some nilpotent distributions}, J. Dyn. Control Syst. \textbf{23} (2017),
  no.~3, 547--575.
	
\bibitem%[BCC05]
{boscain3level}
Ugo Boscain, Thomas Chambrion, and Gr{\'e}goire Charlot, \emph{Nonisotropic
  3-level quantum systems: complete solutions for minimum time and minimum
  energy}, Discrete Contin. Dyn. Syst. Ser. B \textbf{5} (2005), no.~4,
  957--990 (electronic).
	
\bibitem{buseman}
 H. Busemann,
The Isoperimetric Problem in the Minkowski Plane,
{\em American Journal of Mathematics}, Vol. 69, No. 4 (Oct., 1947), pp. 863--871

\bibitem{S18}
	Yu. L. Sachkov, Optimal bang-bang trajectories in sub-Finsler problem on the Cartan group, Russian Journal of Nonlinear Dynamics, 2018, vol.4, n.4, 583-593. 

\bibitem{(3,6)}
	Yu. L. Sachkov, Periodic controls in step 2 strictly convex sub-Finsler problems,
Regular and Chaotic Dynamics, 2020, Vol. 25, No. 1, pp. 33--39.

\subsection*{Левоивариантные сублоренцевы задачи}
\bibitem{CHSY}
Qihui Cai, Tiren Huang, Yu. Sachkov, Xiaoping Yang, Geodesics in the Engel group with a sub-Lorentzian metric, {\em Journal of Dynamical and Control Systems}, Vol. 22 (2016), 465--484.

\bibitem{ASHY}
А. А. Ардентов, Ю. Л. Сачков, Т. Хуанг, К. Янг, “Экстремальные траектории в сублоренцевой задаче на группе Энгеля”, Матем. сб., 209:11 (2018), 3–31

\subsection*{Разные статьи по левоивариантным задачам} 

\bibitem{BBG}
Davide Barilari, Ugo Boscain, and Jean-Paul Gauthier. On 2-step,
corank 2 sub-Riemannian metrics. SIAM J. Control Optim., 50(1):
559–582, 2012.

\bibitem{BCG}
U. Boscain, T. Chambrion, and J.-P. Gauthier. On the K + P problem
for a three-level quantum system: optimality implies resonance. J. Dyn.
Control Syst., 8(4): 547–572, 2002.

\bibitem{brock99}
Roger W Brockett. Explicitly solvable control problems with
nonholonomic constraints. In Decision and control, 1999, Proc.
38th IEEE Conf. on, volume 1, pp. 13–16. IEEE, 1999.


\bibitem{ber18}
В. Н. Берестовский, “Геодезические и кривизны специальных субримановых метрик на группах Ли”, Сиб. матем. журн., 59:1 (2018), 41–55 

\bibitem{ber14}
В. Н. Берестовский, “Универсальные методы поиска нормальных геодезических на группах Ли с левоинвариантной субримановой метрикой”, Сиб. матем. журн., 55:5 (2014), 959–970 

\bibitem{MS15}%!
	А.П. Маштаков, Ю.Л. Сачков, Суперинтегрируемость левоинвариантных субримановых структур на унимодулярных трехмерных группах Ли, Дифференциальные уравнения, 2015, 11, 1482—1488.

\subsection*{Нильпотентная аппроксимация и конструктивное решение задачи управления}
\bibitem{agrach_sarych}
%A.\,A.~Agrachev, A.\,A.~Sarychev,
%Filtration of a Lie algebra of vector fields and nilpotent
%approximation of control systems,
%{\em Dokl. Akad. Nauk SSSR}, {\bf 295} (1987),
%English transl. in {\em Soviet Math. Dokl.}, {\bf 36} (1988),
%104--108.
Аграчев А.А., Сарычев А.А.
Фильтрация алгебры Ли векторных полей и нильпотентная аппроксимация управляемых
систем//
Докл. АН СССР.
1987.
Т. 295, No. 4, С. 777–781

\bibitem{masht12}
А. П. Маштаков, Алгоритмическое и программное обеспечение решения
конструктивной задачи управления неголономными пятимерными
системами, Программные системы: теория и приложения, 3:1 (2012),
с. 3–29



\bibitem{agrachev_marigo}
A. Agrachev and A. Marigo. Nonholonomic tangent spaces: intrinsic
construction and rigid dimensions. Electron. Res. Announc. Amer. Math.
Soc., 9: 111–120, 2003.

\bibitem{bellaiche}
Bellaiche A.
The tangent space in sub-Riemannian geometry//
In: Sub-Riemannian geometry, A.~Bellaiche and J.-J.~Risler,
Eds., Birkh\"auser, Basel, Swizerland, 1996, 1--78.

\bibitem{Bellaiche11}  
{\it Bellaiche~A., Laumond~J. P., Chyba~M.}
Canonical nilpotent approximation of control systems: application to nonholonomic motion planning. 32nd IEEE CDC, 1993.

\bibitem{Bellaiche10} 
{\it Bellaiche~A., Laumond~J.P., Risler~J.J.}
Nilpotent infinetisimal approximations to a control Lie algebra. IFAC NCSDS, Bordeaux, 1992. P.~174--181.

\bibitem{BS}
Rosa Maria Bianchini and Gianna Stefani. Graded approximations
and controllability along a trajectory. SIAM J. Control Optim., 28(4):
903–924, 1990.

\bibitem{Jean2013}
{\it Chitour~Y., Jean~F., Long~R.}
A Global Steering Method for Nonholonomic Systems, Journal of Differential Equations, 2013, V. 254, P. 1903--1956.

\bibitem{Fer35} {\it Fernandes~C., Gurvits~L., Li~Z.X.} 
A variational approach to optimal nonholonomic motion planning. IEEE ICRA, Sacramento, 1991. P. 680--685.

\bibitem{gromov}
Mikhael Gromov. Carnot–Carath\'eodory spaces seen from within. In
Sub-Riemannian geometry, volume 144 of Progress in Mathematics,
pp. 79–323. Birkh\"auser, Basel, 1996.

\bibitem{b:hermes}
{\it Hermes H.}
Nilpotent and high-order approximations of vector fields systems //  SIAM. 1991. V. 33. P. 238--264.

\bibitem{b:lafsus}
{\it Lafferriere~G., Sussmann~H.J.}
A differential geometric approach to motion planning. 
Nonholonomic Motion Planing. 1992. Editors: Zexiang Li, J.F. Canny.

\bibitem{suss2}
Laferriere, G. and Sussmann, H.J., A differential geometric approach to motion planning, \textit{Nonholonomic motion planning}, Kluwer, 1993, pp.~235--270.

\bibitem{laumond}
Laumond J.P.
Nonholonomic motion planning for mobile robots// Preprint No.~98211.
 Toulouse, France: LAAS-CNRS, 1998.

\bibitem{l81} Murray R. M., {\em Nilpotent bases for a class on nonintegrable distributions with applications to trajectory generation for nonholonomic systems}// Math. Control Signal Syst., university of California, Berkeley, 1990.

\bibitem{stefani}
{\it Stefani G.}
Polynomial approximations to control systems and local controllability // Proc. 24th. I.E.E.E. Conference on Decision and
Control, Ft. Lauderdale, Fla., 1985, P. 33--38.

\bibitem{TilSas119} Tilbury D., Murray R., Sastry S., {\em Trajectory generation for the n-trailer problem using Goursat normal form}// IEEE TAC, 1995, V. 40, No. 5, P. 802--819.

\bibitem{vendit_laumond_oriolo}
Vendittelli M., Laumond J.P., Oriolo G.
Steering nonholonomic systems via nilpotent approximations: The general two-
trailer
system//
1999 IEEE International Confer. on Robotics and Automation, May 10--15,
1999,
Detroit, MI.

\bibitem{b:venditelli}
{\it Venditelli~M., Oriolo~G., Jea~F., Laumond~J.P.}
Nonhomogeneous nilpotent approximations for nonholonomic systems with singularities // Transactions on Automatic Control. 2004. P. 261--266.

\bibitem{walsh}
Walsh, G.C., Montgomery, R., and Sastry, S.S., Optimal path planning on matrix Lie group, in \textit{Proc. of the 33rd IEEE Conference on Decision and Control}, 1994, vol.~2, pp.~1258--1263. 


\subsection*{Приложения субримановой геометрии к моделям зрения и обработке изображений}
\bibitem{MDSBB}
	А. П. Маштаков, P. Дайтс, Ю. Л. Сачков, E. Беккерс, И. Ю. Бесчастный, Субримановы геодезические на группе SO(3) в задаче поиска кровеносных сосудов на сферических изображениях сетчатки,  Доклады Академии Наук, 2017, 473, № 5, с. 521–524

\bibitem{benyosef}
G.~Ben-Yosef and O.~Ben-Shahar, {\em A tangent bundle theory for visual
curve completion}. PAMI 34(7), pp.1263–-1280, 2012.

\bibitem{BDMG15}
E .J. Bekkers, R. Duits, A. Mashtakov, G. R. Sanguinetti. “A PDE approach
to data-driven sub-Riemannian geodesics in SE(2)”, SIAM Journal on
Imaging Sciences, 8:4 (2015), pp. 2740–2770

\bibitem{BDMS17}
E. J. Bekkers, R. Duits, A. Mashtakov, Y. Sachkov. “Vessel tracking via
sub-Riemannian geodesics on the projective line bundle”, Geometric Science
of Information, GSI 2017, LNCS, vol. 10589, eds. F. Nielsen, F. Barbaresco,
Springer, Cham, 2017, pp. 773–781.

\bibitem{Boscain2014}
U.~Boscain, R.~Duits, F.~Rossi and Y.~L.~Sachkov,
Curve Cuspless Reconstruction via sub-Riemannian Geometry,
ESAIM: Control, Optimisation and Calculus of Variations, 20 (2014), 748--770,
doi:10.1051/cocv/2013082

\bibitem{Gauthier}
U. Boscain, J.-P. Gauthier, R. Chertovskih, A. Remizov
Hypoelliptic diffusion and human vision: a semidiscrete new twist //
SIAM J. Imaging Sci., 7 (2), 2014, pp. 669--695.

\bibitem{citti_sarti}
G. Citti, A. Sarti. A cortical based model of perceptual completion in the
roto-translation space, Journal of Mathematical Imaging and Vision, 24:3
(2006), pp. 307–326.

\bibitem{DuitsJMIV2014}
R.~Duits, U.~Boscain, F.~Rossi and Y.~L.~Sachkov,
Association Fields via Cuspless Sub-Riemannian Geodesics in SE(2) //
JMIV, 49 (2), 2014, pp. 384--417, doi: 10.1007/s10851-013-0475-y

\bibitem{DuitsIJCV2007}
R.~Duits, M.~Felsberg, G.~Granlund, B.H.~Romeny, {\em Image Analysis and Reconstruction using a Wavelet Transform Constructed from a Reducible Representation of the Euclidean Motion Group.} IJCV, vol.72 (1), pp. 79--102, 2007.

\bibitem{JDCS16}
R.~Duits, A.~Ghosh,  T.\,C.\,J.~Dela Haije, A.~Mashtakov,
On Sub-Riemannian Geodesics in SE(3) Whose Spatial Projections do not Have Cusps // Journal of Dynamical and Control Systems, 2016, 22(4), pp:771--805, doi:10.1007/s10883-016-9329-4

\bibitem{FMCS}
B. Franceschiello, A. Mashtakov, G. Citti, A. Sarti. “Modelling of the
Poggendorff illusion via sub-Riemannian geodesics in the roto-translation
group”, New Trends in Image Analysis and Processing, ICIAP 2017, LNCS,
vol. 10590, eds. S. Battiato, G. M. Farinella, M. Leo, G. Gallo, Springer,
2017, pp. 37–47.

\bibitem{DGA19}
B. Franceschiello, A. Mashtakov, G. Citti, A. Sarti, Geometrical optical illusion via sub-Riemannian geodesics in the roto-translation group // Differential Geometry and its Applications, Volume 65, 2019, pp. 55--77, doi:10.1016/j.difgeo.2019.03.007

\bibitem{Franken2009}
E.~Franken and R.~Duits,
{\em Crossing-Preserving Coherence-Enhancing Diffusion on Invertible Orientation Scores.}
IJCV, 85(3), pp. 253-278, 2009.

\bibitem{MAS13}
A. P. Mashtakov, A. A. Ardentov, Yu. L. Sachkov. “Parallel algorithm
and software for image inpainting via sub-Riemannian minimizers on the
group of rototranslations”, Numerical Mathematics: Theory, Methods and
Applications, 6:1 (2013), pp. 95–115.

\bibitem{MDSBB17}
A. Mashtakov, R. Duits, Y. Sachkov, E. J. Bekkers, I. Beschastnyi. “Tracking
of lines in spherical images via sub-Riemannian geodesics in SO(3)”, JMIV,
58:2 (2017), pp. 239–264

\bibitem{petitot}
J.Petitot, The neurogeometry
	of pinwheels as a sub-Riemannian contact structure, 
	{\em J. Physiology - Paris} 97 (2003), 265--309.

\bibitem{petitot_book}
J.Petitot, 
{\em Neurogeometrie de la vision --- Modeles mathematiques et physiques des architectures fonctionnelles}, 2008, Editions de l'Ecole Polytechnique. 

\subsection*{Приложения субримановой геометрии к робототехнике}
\bibitem{Ar-Eu-mob-rob} А. А. Ардентов, А. В. Смирнов, Управление мобильным роботом вдоль эластик Эйлера, Программные системы: теория и приложения, 2017, том 8, выпуск 4, 163–178

\bibitem{markov}
А.А. Марков, Несколько примеров решения особого рода задач о наибольших и наименьших величинах // Сообщ. Харьков. матем. общ. Вторая сер., 1:2 (1889), 250–276.

\bibitem{ArdentovRCD}
{\it Ardentov A.A.} 
Controlling of a mobile robot with a trailer and its nilpotent approximation // Regular and Chaotic Dynamics. 2016. V. 21. No. 7--8, P. 775--791.

\bibitem{EU-robot}
Ardentov A.A., Karavaev Y.L., Yefremov K.S.
Euler Elasticas for Optimal Control of the Motion of Mobile Wheeled Robots: the Problem of Experimental Realization // RCD.
2019. V. 24. No. 3. P. 312--328.

\bibitem{dubins}
{\it Dubins L.E.}
On curves of minimal length with a constraint on average curvature, and with prescribed initial and terminal positions and tangents // American Journal of Mathematics. 1957. V. 79. No. 3. P. 497--516.

\bibitem{laum98}
Laumond, J.-P., \textit{Nonholonomic motion planning for mobile robots}, Tutorial notes, 1998.

\bibitem{sussmann_tang}
Sussmann, H.J. and Tang, G., Shortest paths for the Reeds-Shepp car: a~worked out example of the use of geometric techniques in nonlinear optimal control, \textit{Report SYCON-91-10}, 1991.

\bibitem{reeds}
Reeds, J.A. and Shepp, L.A., Optimal paths for a car that goes both forwards and backwards, \textit{Pacific J. Math.}, 1990. vol.~145, no.~2, pp.~367--393.

\end{thebibliography}

